Learning Where and How Much to Sample: Volume-Adaptive k-Space Acquisition for Accelerated MRI

Magnetic resonance imaging (MRI) is an essential medical imaging technique, but its high costs and long acquisition times can limit accessibility. Accelerated MRI reduces acquisition time through k-space undersampling, yet conventional methods often rely on predefined sampling patterns and uniform slice budgets, overlooking anatomical variations and inter-slice relationships. In this paper, we propose a volume-adaptive k-space acquisition framework that jointly learns where and how much to sample across an entire MRI volume. Using only acquired auto-calibration signal (ACS) measurements, our method exploits volume-wide anatomical information to adaptively allocate sampling budgets across slices while identifying informative k-space lines. A learned joint slice--frequency refinement module coordinates sampling decisions while preserving an exact total volume-level acquisition budget. To reconstruct the acquired measurements, we design a sensitivity-aware synchronous cross-slice reconstruction network that estimates coil sensitivities from ACS measurements and progressively refines neighboring-slice reconstructions while enforcing hard k-space data consistency. Both networks are jointly optimized using reconstruction-based supervision without requiring fully sampled k-space at inference. Experiments on knee and brain MRI across multiple contrasts and acceleration factors demonstrate the adaptive behavior of our acquisition framework and evaluate its reconstruction performance.

==> Figure_MRI/Figure_Pipeline.tex <==

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figure_MRI/Pipeline.png}
    \caption{
    Workflow of the proposed adaptive MRI scanning procedure. 
    Initial multi-coil ACS measurements guide
    adaptive k-space selection. The scanner then acquires
    additional informative lines, and our reconstruction
    network recovers the final MRI image.
    }
    \label{fig:pipeline}
    \vspace{-2mm}
\end{figure}


==> Figure_MRI/Figure_brain.tex <==

% Requires graphicx and booktabs.
% Add this helper only once in your document.

\providecommand{\brainpanel}[2]{%
    \IfFileExists{#1}{%
        \includegraphics[
            width=0.115\textwidth,
            height=#2,
            keepaspectratio
        ]{#1}%
    }{%
        \fbox{%
            \parbox[c][#2][c]{0.105\textwidth}{%
                \centering\tiny Pending%
            }%
        }%
    }%
}

\begin{figure*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}

\begin{tabular}{lccccccc}
\toprule
& \textbf{GT}
& \textbf{Adjoint}
& \textbf{Scalar TV}
& \textbf{Adaptive TV}
& \textbf{SwinIR}
& \textbf{MoDL}
& \textbf{VOSAR (Ours)} \\
\midrule

% ==========================
% T1
% ==========================

\textbf{T1}
& \brainpanel{figures/brain/t1/gt.png}{2.0cm}
& \brainpanel{figures/brain/t1/adjoint.png}{2.0cm}
& \brainpanel{figures/brain/t1/scalar_tv.png}{2.0cm}
& \brainpanel{figures/brain/t1/adaptive_tv.png}{2.0cm}
& \brainpanel{figures/brain/t1/swinir.png}{2.0cm}
& \brainpanel{figures/brain/t1/modl.png}{2.0cm}
& \brainpanel{figures/brain/t1/ours.png}{2.0cm}
\\

\textbf{Mask}
& --
& \brainpanel{figures/brain/t1/adjoint_mask.png}{0.9cm}
& \brainpanel{figures/brain/t1/scalar_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/t1/adaptive_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/t1/swinir_mask.png}{0.9cm}
& \brainpanel{figures/brain/t1/modl_mask.png}{0.9cm}
& \brainpanel{figures/brain/t1/ours_mask.png}{0.9cm}
\\

\midrule

% ==========================
% T2
% ==========================

\textbf{T2}
& \brainpanel{figures/brain/t2/gt.png}{2.0cm}
& \brainpanel{figures/brain/t2/adjoint.png}{2.0cm}
& \brainpanel{figures/brain/t2/scalar_tv.png}{2.0cm}
& \brainpanel{figures/brain/t2/adaptive_tv.png}{2.0cm}
& \brainpanel{figures/brain/t2/swinir.png}{2.0cm}
& \brainpanel{figures/brain/t2/modl.png}{2.0cm}
& \brainpanel{figures/brain/t2/ours.png}{2.0cm}
\\

\textbf{Mask}
& --
& \brainpanel{figures/brain/t2/adjoint_mask.png}{0.9cm}
& \brainpanel{figures/brain/t2/scalar_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/t2/adaptive_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/t2/swinir_mask.png}{0.9cm}
& \brainpanel{figures/brain/t2/modl_mask.png}{0.9cm}
& \brainpanel{figures/brain/t2/ours_mask.png}{0.9cm}
\\

\midrule

% ==========================
% FLAIR
% ==========================

\textbf{FLAIR}
& \brainpanel{figures/brain/flair/gt.png}{2.0cm}
& \brainpanel{figures/brain/flair/adjoint.png}{2.0cm}
& \brainpanel{figures/brain/flair/scalar_tv.png}{2.0cm}
& \brainpanel{figures/brain/flair/adaptive_tv.png}{2.0cm}
& \brainpanel{figures/brain/flair/swinir.png}{2.0cm}
& \brainpanel{figures/brain/flair/modl.png}{2.0cm}
& \brainpanel{figures/brain/flair/ours.png}{2.0cm}
\\

\textbf{Mask}
& --
& \brainpanel{figures/brain/flair/adjoint_mask.png}{0.9cm}
& \brainpanel{figures/brain/flair/scalar_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/flair/adaptive_tv_mask.png}{0.9cm}
& \brainpanel{figures/brain/flair/swinir_mask.png}{0.9cm}
& \brainpanel{figures/brain/flair/modl_mask.png}{0.9cm}
& \brainpanel{figures/brain/flair/ours_mask.png}{0.9cm}
\\

\bottomrule
\end{tabular}

\caption{
Qualitative reconstruction comparisons on the M4Raw
low-field brain MRI dataset at $4\times$ acceleration.
Representative T1-weighted, T2-weighted, and FLAIR
examples are shown.
For each contrast, the upper row presents reconstructed
images and the lower row shows the corresponding
k-space sampling masks.
We compare Adjoint, Scalar TV, Adaptive TV, SwinIR,
and MoDL with the proposed VOSAR framework.
All comparisons use matched total acquisition budgets
and the same reference image for each example.
}
\label{fig:m4raw_qualitative}

\end{figure*}


==> Sec_MRI/Statement.tex <==
\section*{LLM Usage Statement}
OpenAI ChatGPT was used to assist with experimental implementation, language editing, and the preparation of illustrative figures.
%
The authors reviewed all AI-generated content and remain responsible for the scientific accuracy and integrity of the work.

==> Table_MRI/Table_ablation.tex <==

\begin{table*}[t]
\centering
\caption{
Ablation study of the proposed framework at $8\times$
acceleration on fastMRI Knee and M4Raw Brain.
PSNR (dB) and SSIM (\%) are reported under matched
acquisition budgets.
}
\label{tab:ablation}
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l*{6}{c}}
\toprule
& \multicolumn{2}{c}{Knee PD}
& \multicolumn{2}{c}{Knee PDFS}
& \multicolumn{2}{c}{M4Raw Brain} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Configuration
& PSNR$\uparrow$ & SSIM$\uparrow$
& PSNR$\uparrow$ & SSIM$\uparrow$
& PSNR$\uparrow$ & SSIM$\uparrow$ \\
\midrule

w/o Adaptive Slice Budgets
& -- & -- & -- & -- & -- & -- \\

w/o Learned Frequency Selection
& -- & -- & -- & -- & -- & -- \\

w/o Volume-Level ACS Modeling
& -- & -- & -- & -- & -- & -- \\

w/o Joint Slice--Frequency Refinement
& -- & -- & -- & -- & -- & -- \\

w/o Contrast Conditioning
& -- & -- & -- & -- & -- & -- \\

w/o Cross-Slice Reconstruction
& -- & -- & -- & -- & -- & -- \\

\midrule
\textbf{Full Model (Ours)}
& -- & -- & -- & -- & -- & -- \\

\bottomrule
\end{tabular*}
\end{table*}


==> Table_MRI/Table_inference.tex <==

\begin{table*}[t]
\centering
\caption{
Inference efficiency comparison on the fastMRI
multi-coil knee dataset at $8\times$ acceleration.
All methods are evaluated on the same volumes
using identical hardware and inference settings.
Sampling time includes ACS-based acquisition
planning, while reconstruction time measures
neural network inference.
Total time excludes physical MRI acquisition.
PSNR is reported separately for PD and PDFS.
}
\label{tab:inference_efficiency}

\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular*}{\textwidth}{
@{\extracolsep{\fill}}lcccccc
}
\toprule
& \multicolumn{2}{c}{Reconstruction Quality}
& \multicolumn{3}{c}{Inference Time (s/volume)}
& Peak GPU \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-6}
Method
& PD PSNR$\uparrow$
& PDFS PSNR$\uparrow$
& Sampling
& Reconstruction
& Total$\downarrow$
& Memory (GB)$\downarrow$ \\
\midrule

U-Net
& -- & -- & -- & -- & -- & -- \\

i-RIM
& -- & -- & -- & -- & -- & -- \\

E2E-VarNet
& -- & -- & -- & -- & -- & -- \\

HUMUS-Net
& -- & -- & -- & -- & -- & -- \\

PromptMR
& -- & -- & -- & -- & -- & -- \\

PromptMR+
& -- & -- & -- & -- & -- & -- \\

\midrule

VOSAR w/o Adaptive Budgets
& -- & -- & -- & -- & -- & -- \\

VOSAR w/o Volume Coordination
& -- & -- & -- & -- & -- & -- \\

\textbf{VOSAR (Ours)}
& -- & -- & -- & -- & -- & -- \\

\bottomrule
\end{tabular*}
\end{table*}

